Robust Safety under Stochastic Uncertainty with Discrete-Time Control Barrier Functions

Robots deployed in unstructured, real-world environments operate under considerable uncertainty due to imperfect state estimates, model error, and disturbances. Given this real-world context, the goal of this paper is to develop controllers that are provably safe under uncertainties. To this end, we leverage Control Barrier Functions (CBFs) which guarantee that a robot remains in a ``safe set'' during its operation -- yet CBFs (and their associated guarantees) are traditionally studied in the context of continuous-time, deterministic systems with bounded uncertainties. In this work, we study the safety properties of discrete-time CBFs (DTCBFs) for systems with discrete-time dynamics and unbounded stochastic disturbances. Using tools from martingale theory, we develop probabilistic bounds for the safety (over a finite time horizon) of systems whose dynamics satisfy the discrete-time barrier function condition in expectation, and analyze the effect of Jensen's inequality on DTCBF-based controllers. Finally, we present several examples of our method synthesizing safe control inputs for systems subject to significant process noise, including an inverted pendulum, a double integrator, and a quadruped locomoting on a narrow path.

==> constant_d_proof.tex <==
\begin{proof}
    To prove this theorem, we will rely on Ville's Inequality. In order to do that we must first construct, a nonnegative super martingale. 
    For this purpose consider the candidate function $W: \R^n \times \mathbb{N}_\geq 0 \to \R^n  $: 
    \begin{align}
        W(\mb{x}_k, k) & \triangleq \underbrace{ \theta^{k} ( M - h(\mb{x}_k)) } _{\textrm{negate and rescale}} - \underbrace{e \sum_{i=0}^n \theta^i }_{\textrm{cancel }e} + \underbrace{e \sum_{i=0}^K \theta^i }_{\textrm{ensure nonegativity}}  \\%\underbrace{\frac{\gamma + M}{K^N}}_{\textrm{ensure nonnegativity}}.\
        & = \theta^k (M - h(\mb{x}_k) ) - e \left( \frac{1 -\theta^{k+1} }{1 - \theta } - \frac{1 - \theta^{K+1}}{1 - \theta }\right)\\
        & = \theta^k (M - h(\mb{x}_k) - \frac{e\theta^{k+1}}{\theta -1 } + \frac{e\theta^{K+1}}{\theta - 1 }
    \end{align}
    Where the identity for a geometric series was used. Also,  $e \triangleq  M(1-\alpha) - d $ and $\theta \in \R_{>1}$ is a free variable which will be used later to optimize the bound on $P_u$. Since $e$ is greater than or equal to zero and $h$ is upper bounded by $M$, $W$ is nonnegative. 

    
    
    
    Next we must show that $W(\mb{x}_n, n)$ satisfies the super-martingale inequality: 
    \begin{align}
        & \mathbb{E}[W(\mb{x}_{k+1}, k+1) ~|~ (\mb{x}_k, k)] \nonumber \\
        & = (M- \E[h(\mb{x}_{k+1})~|~ x_k])\theta^{k+1}   - \frac{e\theta^{k+2}}{\theta - 1} + \frac{e \theta^{K+1}}{\theta - 1}\\
        & \leq  (M - \alpha h(\mb{x}_k) - d_k )\theta^{k+1}  - \frac{e\theta^{k+2}}{\theta - 1} + \frac{e \theta^{K+1}}{\theta - 1} \\
        & = \alpha \theta (M - h(\mb{x}_k) )\theta^{k}  - \frac{e\theta^{k+2}}{\theta - 1} + \frac{e \theta^{k+1}}{\theta - 1} + e \theta^{k+1} \\
        & \leq  (M - h(\mb{x}_k) )\theta^{k}  + \frac{e\theta^{K+1}}{(\theta - 1)} + \theta^{k+1} \left( e - \frac{e\theta }{\theta - 1} \right)  \\
        & =  (M - h(\mb{x}_k) )\theta^{k}  - \frac{e\theta^{k+1}}{(\theta - 1) }+ \frac{e\theta^{K+1}}{(\theta - 1)}  \\
        & = W(\mb{x}_k, k) 
    \end{align}
    Here we required that $\theta \leq \frac{1}{\alpha }$. Thus, if $\theta \in (0, 1/\alpha ]\setminus\{1\} $, then $W(\mb{x}_n, n) $ is a nonnegative super-martingale. 
    %Note that since $\alpha \in (0,1)$ $\gamma\geq 0$, and $M>0$,  $ [\alpha, \frac{\alpha M + \gamma }{M + \gamma  } ] $ is non-empty. 
    
    Since we have shown that $W(\mb{x}_n, n) $ is a nonnegative super-martingale, we can apply Ville's Inquality: 
    \begin{align}
        \mathbb{P}\left\{\max_{0\leq n \leq N} W(\mb{x}_n, n) \geq \lambda \right\}\leq \frac{M - h(\mb{x}_0) - \frac{e \theta}{\theta - 1}  + \frac{e\theta^{K+1}}{\theta -1}}{\lambda}
    \end{align}
    
    Now we must relate level sets of $W(\mb{x}_n, n) $ to level sets of $h$. In particular, to bound $P_u$ we require that $\min_{n \in \{0, \dots, N\} } h(\mb{x}_n) \leq -\gamma $ implies that $\max_{n \in \{0, \dots, N\}}W(\mb{x}_n, n) \geq \lambda $. 
    \begin{align}
        &\max_{k \in \{0, \dots, N\}}  W(\mb{x}_n, n) -\lambda \nonumber\\
        & = \max_{k \in \{0, \dots, N\}} (M- h(x_k)) \theta^{k} - \frac{e\theta^{k+1}}{\theta -1} + \frac{e\theta^{K+1}}{\theta -1 } - \lambda \\
        & \geq   -\theta^\kappa\min_{k \in \{0, \dots, N\}} h(\mb{x}_k)  + \theta^\kappa \min  \underbrace{\left( \frac{M + \frac{e\theta^{K+1}}{\theta-1}- \lambda }{\theta^k} + \frac{-e\theta}{\theta -1 }  \right) }_{\triangleq r(k, \theta) } 
    \end{align}
    To lowerbound this we seek to choose $\theta$ and $\lambda$ such that $\min_{k} r(k, \theta) \geq  -\gamma$. Since $\theta >1$, $r(k, \theta) $ achieves its minimum at $k^*=0$ when $(M + \frac{e\theta^{K+1}}{\theta -1} - \lambda ) \geq 0  $ and at $k^* =K$ when $(M + \frac{e\theta^{K+1}}{\theta -1} - \lambda ) \leq 0 $.
    
    In particular, we choose: 
    \begin{align}
        \lambda = \gamma \theta^{k^*} + M + \frac{e\theta^{K+1}}{\theta -1} - \frac{e\theta^{k^*+1}}{\theta -1},
    \end{align}
    where $k^* $ minimizes $r(k,\theta) $ for a particular $\theta$. 

    
    %By choosing $\lambda$ and $\theta$ such that $M  + \frac{e\theta^{K+1}}{\theta-1} > \lambda  $, the minimum occurs at $k^* = K$ and by choosing $F(K, \theta) < \lambda $, the minimum occurs at $k^* = 0 $ since $F(k, \theta)$ grows monotonically in $k$. 
    % To lowerbound this we choose $\lambda = (\gamma + M)K^{-N} $ such that $r(n) =0 $ for all $n$. This ensures that $-h(\mb{x}_n) - \gamma \geq 0 \implies -\gamma -h(\mb{x}_n) + r(n) \geq 0 $ for all $n$. Furthermore since $\frac{1}{K^n } >1 $ for all $n$,  
    %If $M\alpha^{-N}>\lambda $ then the minimum occurs at $n^* =0 $, if $M\alpha^{-N}<\lambda $ then the minimum occurs at $n^*=N$. 
    % \begin{align}
    %      \max_{n \in \{0, \dots, N\}} W(\mb{x}_n, n) &  - (\gamma + M)K^{-N} \nonumber  \\
    %     & \geq \max_{n \in \{0, \dots, N\}}\underbrace{\left(-\gamma  -h(\mb{x}_n) \right)  }_{\geq 0, \textrm{ by hypothesis}}\\
    %     & =  -\gamma - \min_{n \in \{0, \dots, N\}} (h(\mb{x}_n) %\min_{n \in \{0, \dots, N\}}\left( (\gamma + M) K^{n-N} - \lambda K^n \right) \\
    % \end{align}
    This ensures that
    \begin{align}
        &\min_{n \in \{0, \dots, N\}}    h(\mb{x}_n) \leq -\gamma \nonumber \\
        & \implies \max_{n \in \{0, \dots, N\}}  W(\mb{x}_n, n) \geq \gamma \theta^{k^*} + M + \frac{e\theta^{K+1}}{\theta -1} - \frac{e\theta^{k^*+1}}{\theta -1}
    \end{align}
    
    This allows us to apply the previous bound to $P_u$: 
    \begin{align}
        P_u &\leq \mathbb{P}\left\{\max_{n \in \{0, \dots, N\}} W(\mb{x}_n, n) \geq \lambda \right\}\\
        & \leq  \frac{M - h(\mb{x}_0) - \frac{e \theta}{\theta - 1}  + \frac{e\theta^{K+1}}{\theta -1}}{\gamma \theta^{k^*} + M  - \frac{e\theta^{k^*+1} }{\theta -1}+ \frac{e\theta^{K+1}}{\theta -1}}
    \end{align}

    \textbf{First Case: }$(M + \frac{e\theta^{K+1}}{\theta -1} - \lambda ) \geq 0  $ which ensures that $k^*=0$ is a minimizer. Also, using our choice of minimizing $\lambda$, this means that: 
    \begin{align}
        0 &\leq M + \frac{e\theta^{k+1}}{\theta -1} - \lambda   \\
        & =  M + \frac{e\theta^{k+1}}{\theta -1} - \gamma - M - \frac{e\theta^{K+1}}{\theta -1} + \frac{e\theta}{\theta -1}\\
        \implies & \theta \leq \frac{e + \gamma }{\gamma }
    \end{align}
    In this case, the bound becomes: 
    \begin{align}
        P_u 
        & \leq  \frac{M - h(\mb{x}_0) - \frac{e \theta}{\theta - 1}  + \frac{e\theta^{K+1}}{\theta -1}}{\gamma + M  - \frac{e\theta }{\theta -1}+ \frac{e\theta^{K+1}}{\theta -1}}\\
        & = \frac{M - h(\mb{x}_0) +\frac{e\theta }{\theta -1}( \theta^{K} -1)}{\gamma + M  + \frac{e\theta }{\theta -1}( \theta^{K} -1)}
    \end{align}


    \textbf{Consider the first case} where $\theta F(K, \theta) \leq \lambda  $ and $k^* = 0 $. This bound becomes: 
    \begin{align}
        P_u &  \leq  \frac{M - h(\mb{x}_0)  - \theta + \theta F(K, \theta)}{F(0, \theta) (M - \theta + \gamma) + \theta F(K, \theta)} \\
        & = \frac{M - h(\mb{x}_0)  + \theta( F(K, \theta)-1) }{M + \gamma + \theta(  F(K, \theta) -1)   } 
    \end{align}
    Since $\theta F(K, \theta) - \lambda \leq  0 $  and $\lambda = (M - \theta + \gamma) + \theta F(K, \theta)$, we require that $\theta \in [\overline{e} / (1 - \alpha),  M + \gamma] $. This bound shrinks as $\theta$ increases, so we choose $\theta = M+\gamma$ to achieve the bound: 
    \begin{align}
        P_u &\leq \frac{M - h(\mb{x}_0) + (M+\gamma)(F(K, \theta) -1) }{(M+\gamma) F(K, \theta)  }\\
        & = 1 - \frac{h(\mb{x}_0) + \gamma }{(M + \gamma)F(K, \theta) }\\
        & = 1 - \frac{h(\mb{x}_0) + \gamma }{M+\gamma}\prod_{i=0}^{K-1} \left(  \frac{M+\gamma -e_i}{M+ \gamma} \right) \\
        & = 1 - \frac{h(\mb{x}_0) + \gamma }{M+\gamma}\prod_{i=0}^{K-1} \left(  \frac{M\alpha +\gamma +d_i}{M+ \gamma} \right) 
    \end{align}

    In this case, 
    \begin{align}
        \frac{M(1- \alpha) + \overline{d}}{(1-\alpha)} \leq M + \gamma
    \end{align}
    \textbf{Consider the second case} where $\theta F(K, \theta) > \lambda $ and $k^* = K$. The bound becomes: 
    \begin{align}
        P_u &  \leq  \frac{M - h(\mb{x}_0)  - \theta + \theta F(K, \theta)}{F(K, \theta) (M - \theta + \gamma) + \theta F(K, \theta)} \\
        & = \frac{M - h(\mb{x}_0)  + \theta( F(K, \theta)-1) }{(M+ \gamma) F(K, \theta)} \\
        & = \frac{M- h(\mb{x}_0) }{M + \gamma}\frac{1}{F(K, \theta) } + \frac{\theta(F(K, \theta) -1)}{(M + \gamma) F(K, \theta) }
    \end{align}
    
    This bound decreases as $\theta$ decreases, so we choose the smallest value given our previous stipulation that $\theta \geq \max \{ e_k / (1 - \alpha), \lambda / F(K, \theta) \} $ for all $k$. Since $\lambda < 0$ in this case, let $\theta = \overline{e} / (1 - \alpha) $. In this case, $F(K, \frac{\overline{e}}{(1-\alpha) })  = \prod_{i=0}^{K-1}\frac{\overline{e}}{\overline{e} - e_i(1- \alpha) } $ and $ 1 / F(K, \theta) = \prod_{i=0}^{K-1} \left( 1 - \frac{e_i(1-\alpha) }{\overline{e}}\right) $ 
    \begin{align}
        P_u  \leq & \frac{M- h(\mb{x}_0) }{M + \gamma}\frac{1}{F(K, \theta) } + \frac{\theta(F(K, \theta) -1)}{(M + \gamma) F(K, \theta) }\\
        = &  \frac{M- h(\mb{x}_0) }{M + \gamma} \prod_{i=0}^{K-1} \left( 1 - \frac{e_i(1-\alpha) }{\overline{e}}\right) \\
        & \quad + \frac{(M(1-\alpha) + \overline{d})}{(1-\alpha)(M + \gamma) }\left( 1 - \prod_{i=0}^{K-1} \left( 1 - \frac{e_i(1-\alpha) }{\overline{e}}\right)\right) 
    \end{align}
    In this case, from the $\lambda $ equality with $\gamma$, 
    \begin{align}
        \frac{M(1-\alpha) + \overline{d}}{(1- \alpha) } > M + \gamma
    \end{align}

    To finish the proof, flip the implications to get the contrapositive of the cases. 
    % To complete the proof, we must identify the optimal value of $\theta \in (e_k/(1-\alpha), \infty)$.
    % %Since $\alpha \in (0,1)$ this requires that $\lambda \geq M \alpha^{-N}$, so that $r(n) $ can take on nonpositive values. 
    % % In the case that $\lambda > M\alpha^{-N}$, the $\min_{n \in \{0, \dots, N\}} r(n)$  must occur at $n^* = 0$, so $ \lambda = M\alpha^{-N} + \gamma $. Additionally, $\lambda =  M\alpha^{-N}$ implies that $\gamma =0 $. Therefore, for all $\gamma > 0$, 
    % % \begin{align}
    % %     \lambda = M\alpha^{-N} + \gamma, 
    % % \end{align}
    % Since this bound decreases as $K$ increases and we previously required $K \in \left[\alpha, \frac{\alpha M + \gamma}{ M + \gamma }\right]$, we choose $K = \frac{ \alpha M + \gamma}{ M + \gamma }$ to achieve the tightest inequality. This results in the final bound: 
    % \begin{align}
    %     P_u 
    %     &  \leq 1 -  \frac{ (h(\mb{x}_0) + \gamma )  }{ M + \gamma }\left(\frac{  \alpha M + \gamma }{ M + \gamma  }\right)^N
    % \end{align}
\end{proof}

==> old_stuff.tex <==
% \preston{Quick comment before making big edits -- I think we should tread carefully around the stochastic stuff here since we're presenting it as background/motivation. We may want to organize this as: ``vanilla'' discrete-time safety (without disturbances), then bounded (random) disturbances, then our stuff.}
% Standard presentations of Control Barrier Functions assume continuous-time, deterministic, control-affine dynamics of the form: 
% \begin{align}
%     \dot{\mb{x}} = \mb{f}(\mb{x}) + \mb{g}(\mb{x}) \mb{u},
% \end{align}
% where $\mb{f}: \R^n \to \R^n $ and $\mb{g}: \R^n \to \R^{n\times m }$ are locally Lipschitz continuous functions. The control affine assumption made here is valid for a wide variety of systems in continuous-time, including all systems which can be modeled using robotic-manipulator equations.

% These dynamics may have a more complicated relationship with the input, but \cite{taylor_safety_2022} that if $F$ models continuous time dynamics with a Runge-Kutta integrator of the appropriate order than, the discrete-time dynamics are approximately linear in the input. 

% Such a function $h$ is deemed a discrete-time control barrier function (DTCBF) if it satisfies the following property:

% thus ensuring that $h(\mb{x}_k)$, which represents the system's safety, can only decay as fast as the geometric sequence $\alpha^kh(\mb{x}_0) $ which is always positive.

% The DTCBF constraint \eqref{eq:dtcbf_constraint} can be used to verify the safety of an existing controller or it can be included as a constraint in an optimization program to synthesize safe controllers.

% \begin{theorem}[DTCBF Safety \cite{agrawal_constructive_2022}]
%     Let $h$ be a DTCBF for the system \eqref{eq:dt_autonomous}, some $\mathcal{C} \subset \R^n$, and some $\alpha \in [0,1]$. If $\mb{k}: \R^n \to \R^m $ be a continuous function that satisfies \eqref{eq:dtcbf_constraint} for all $\mb{x} \in \mathcal{C}$, then \eqref{eq:dt_autonomous} is safe with respect to $\mathcal{C}$. 
% \end{theorem}

% Unlike the linear constraint of CBFs, the DTCBF constraint \eqref{eq:dtcbf_constraint} (and chance constraints where $\alpha=0$) are not necessarily convex; therefore, it is common to make the additional assumption that $h(\mb{F}(\mb{x}_k, \mb{u}_k)) $ is concave with respect to $\mb{u}_k$ \cite{agrawal2017discrete,ahmadi2019safe,zeng2021safety}. 

% In this section we consider the robustness properties of DTCBFs for systems \eqref{eq:dt_dyn} with bounded disturbances, where $\Vert \mb{d}_k \Vert \leq \delta $ for some $\delta \geq 0$ and all $k \in \mathbb{N}$. 

% One metric for comparing the robustness of safety method is the first exit time.

% Two common perspectives on robustness include first exit time and input-to-state safety (ISSf) \cite{kolathaya2018input}. 

%and some safe set $\mathcal{C} \subset \mathbb{R}^n $ given as the 0-superlevel set of a continuously differentiable function $h: \R^n \to \R$, 

% For the system \eqref{eq:dt_autonomous_dist}, the first escape time with respect to the set $\mathcal{C}$ is: 
% \begin{align}
%     K_{\textrm{esc}} = \inf \{ {k \in \mathbb{N}} ~|~  h(\mb{x}_k) < 0  \}. 
% \end{align}
% In general, we consider systems with larger first escape times to be safer. 
% \begin{definition}[First exit time]
%     For the system \eqref{eq:dt_dyn} governed by a controller $\mb{k}: \R^n \to \R^m $ and some safe set $\mathcal{C} \subset \mathbb{R}^n $ given as the 0-superlevel set of a continuously differentiable function $h: \R^n \to \R$, the first escape time of the system is given as: 
%     \begin{align}
%         K_{\textrm{esc}} = \inf \{ {k \in \mathbb{N}} ~|~  h(\mb{x}_k) < 0  \}
%     \end{align}
% \end{definition}

% In particular they consider expanded sets $\mathcal{C}_\delta \supseteq \mathcal{C}$: 
% \begin{align}
%     \mathcal{C}_\gamma = \{ \mb{x} \in \R^n ~|~ h(\mb{x}) \geq - \gamma \} \label{eq:c_delta}
% \end{align}
% \noindent for some $\gamma > 0$ which are forward invariant in the presence of bounded disturbances. 
% \begin{definition}[Input-to-State Safety (ISSf)]
%     Let $\mathcal{C} \subset \R^n $ be the 0-superlevel set of a continuous function $h: \R^n \to \R$. The system \eqref{eq:dt_dyn} is \textit{input-to-state-safe} (ISSf) if there exists $\delta \geq 0 $ such that $\Vert \mb{d}_k \Vert_\infty  \leq \delta  $ for all $k \in \mathbb{N}$ and there exists a  $\gamma \in \mathcal{K}_\infty $ \footnote{$\gamma \in \mathcal{K}_\infty$ indicates that $\gamma$ is a Class-$\mathcal{K}_\infty$ function. Class-$\mathcal{K}$ are functions $\gamma: \R_{\geq 0 } \to \R_{\geq 0} $ which are radially unbounded \cite{khalil2002nonlinear}.} such that $\mathcal{C}_\delta$ as defined in \eqref{eq:c_delta} is safe. In this case we refer to the set $\mathcal{C}$ as an \textit{input-to-state safe set} (ISSF set). 
% \end{definition}
% \noindent 


% \subsection{Motivating Case: DTCBFs with Bounded Disturbances}
% In this section we motivate our work on stochastic uncertainty with a deterministic example. When $\alpha \in (0,1]$ and $h(\mb{x}_k) > 0$ , the DT-CBF condition is more restrictive than the state constraint $h(\mb{x}_{k+1}) \geq 0 $ . However, in the disturbance-free case ($\Vert \mb{d}_k\Vert_\infty =0$), both ensure the safety of the system with respect to $\mathcal{C}$. This raises the question: 
% \begin{question}
% What is gained by restricting the safety constraint beyond $\alpha = 0$?
% \end{question}
% To analyze the robustness of these systems we start by considering an example which illustrates the effect of $\alpha$ on first exit times. 
% \begin{example}[Effects of $\alpha$ on First Exit Times] 
%     \normalfont
%     For $\mb{x}, \mb{u}, \mb{d} \in \R$, consider the system and set,
%     \begin{align}
%         \mb{x}_{k+1} = \underbrace{\mb{x}_k + 2 + \mb{u}_k}_{\mb{F}(\mb{x}_k, \mb{u}_k)} +~\mb{d} \textrm{ and } \mathcal{C} = \{ \mb{x} ~|~ \underbrace{1-\mb{x}^2}_{h(\mb{x})} \geq 0 \}
%     \end{align}
    % and the controller
    % \begin{align}
    %     \mb{k}(\mb{x}) = \argmin_{\mb{u} \in \R} & \Vert \mb{u} - (2 + \mb{x}_k) \Vert_2^2 \label{eq:example_controller} \\        
    %     \textrm{ s.t. } &  h(F(\mb{x}_k, \mb{u}_k)) \geq \alpha h(\mb{x}_k). \nonumber
    % \end{align}
    % where $\alpha \in [0, 1)$. 

        % For all $\mb{x}\in \mathcal{C}$ this system becomes unsafe in a single step when no input is applied. When $\mb{d}=0$, the controller \eqref{eq:example_controller} enforces the DTCBF constraint \eqref{eq:dtbf_constraint} and thus guarantees the safety of the system according to Theorem \eqref{thm:dtcbf}. When $\mb{d} > 0$, the system can become unsafe in finite time. 

    % Results of simulating this system for $d=0.05$ and $\alpha \in [0, 1)$ can be found in Fig. \ref{fig:example} where it is clear that larger $\alpha$ values led to larger first exit times.  


% One reason for restricting the system to $\alpha > 0$ is that it adds robustness. When $\alpha = 0 $, there always exists a disturbance that can cause a safety violation in a single discrete time step. 

% \begin{proposition} \label{prop:state_constraint_1st_exit_robustness}
%     Consider system \eqref{eq:dt_dyn}. For every $\mb{x}_0 \in \mathcal{C}$ there exists some dynamics $\mb{F}$ and controller $\mb{k}$ that satisfy \eqref{eq:dtcbf_constraint} with $\alpha = 0$ such that $K_\textrm{esc}=1$ for any $\Vert \mb{d}_0 \Vert > 0 $. 
% \end{proposition}
% \noindent The proof is provided in the Appendix \ref{pf:state_constraint_1st_exit_robustness}. When the safety of a DT system with bounded uncertainty is enforced with a state constraint safety may be immediately violated.


% Alternatively when $\alpha  \in (0,1]$, there is increased robustness in exit time: 
% \begin{proposition}\label{prop:dt_cbf_constraint_1st_exit_robustness}
%     Consider system \eqref{eq:dt_dyn}. For every $\mb{x}_0 \in \textrm{Int}(\mathcal{C})$ there exists some disturbance  bound $M_\mb{d} >0$  such that if the dynamics-controller pair $(\mb{F}, \mb{k})$ satisfies \eqref{eq:dtcbf_constraint} with $\alpha >1$, then $\Vert \mb{d}_0 \Vert \leq M_\mb{d}$ implies that $K_\textrm{esc} >1$. 
% \end{proposition}
% \preston{Doesn't this assume the constraint is always feasible? The claim seems correct on its face but spiritually feels like we're saying CBFs solve robust control of every system lol.}
% \noindent The proof is provided in Appendix \ref{pf:dt_cbf_constraint_1st_exit_robustness}. Thus from Propositions \ref{prop:state_constraint_1st_exit_robustness} and \ref{prop:dt_cbf_constraint_1st_exit_robustness} we conclude that the DTCBF constraint guarantees safer (i.e., larger) first exit times for DT systems with bounded uncertainty when $\alpha >0$. Note, however, that this may be at the cost of feasibility for some dynamics. For $\mb{x}_0 \in \textrm{Int}(\mathcal{C})$, the constraint \eqref{eq:dtcbf_constraint} is strictly tighter when $\alpha >0$ than when $\alpha =0$; therefore, increasing $\alpha$ may render \eqref{eq:dtcbf_constraint} infeasible. 

% \begin{theorem}[\label{thm:1st_exit_time}]
%     $K_\textrm{cbf}(0, \mb{x}_0) \leq K_\textrm{cbf}(\alpha, \mb{x}_0) $ for all $\alpha \in [0, 1] $ and all $\mb{x}_0 \in \mathcal{C}$.  
% \end{theorem}
% \noindent The proof in appendix \ref{pf:1st_exit_time} Furthermore, once the system has left the safe set, the state constraint will force the system to immediately re-enter $\mathcal{C}$ which may require a large amount of input, whereas the DT-CBF constraint with $\alpha \in (0,1]$ is a less-strict constraint that enforces an exponential decay in $h$ back towards the safe set $\mathcal{C}$ and allows for inputs to be optimized over a larger set, thus resulting in less required torque during a safety violation. 

% This is because state constraints attempt to force the system to immediately return to $\mathcal{C}$ in a single step whereas DTCBFs with $\alpha > 0 $ attempt to enforce an exponential convergence back to safety. This also likely means that state constraints will require more input since they enforce a stricter constraint. 


%The second robustness property, Input-to-State Safety (ISSf), was originally developed for continuous time CBFs \cite{kolathaya2018input} and is difficult to apply to general DT systems due to the nonlinearity of \eqref{eq:dtcbf_constraint}. Depending on the function $h$, the authors believe that $\mathcal{C}_\delta$ will likely grow with $\alpha \in [0, 1]$, but that when a safety violation occurs more input will be required when $\alpha = 0 $ than when $\alpha >0$. This is due to the 1 step convergence to safety enforced when $\alpha =0$ and the exponential convergence enforced when $\alpha >0$. The ISSf property will be discussed more thoroughly for general stochastic systems in Section \ref{ }. 

% Consider system \eqref{eq:dt_dyn}. If $h$ is Lipschitz continuous with constant $\mathcal{L}_h > 0 $, the dynamics-controller pair $(\mb{F}, \mb{k}) $ satisfies  \eqref{eq:dtcbf_constraint} for some $\alpha \in [0,1)$, and $\Vert \mb{d}_k\Vert \leq M_\mb{d}$ for some $M_\mb{d} >0$, then 
% %with Lipschitz constant $L_h > 0$ and disturbance bound $\delta > 0 $ is ISSf with: 
%     $\mathcal{C}_\gamma = \bigg\{ \mb{x} \in \R^n ~|~ h (\mb{x}) \geq  - \underbrace{\frac{\mathcal{L}_h M_\mb{d} }{(1- \alpha) }}_{\gamma(M_\mb{d})} \bigg \} $
% is forward invariant (ie, safe).

% Alternatively, ISSf is a robustness property which analyzes the degradation of safety in the presence of disturbances by describing the expansion of the set rendered safe:
% \begin{definition}[Input-to-State Safety \cite{kolathaya2018input}]
%     Let $\mathcal{C}\subset\R^n$ be the 0-superlevel set of a continuous function $h:\R^n\to\R$. The system \eqref{eq:dt_autonomous_dist} is said to be input-to-state safe with respect to the set $\C$ if there exists a function $\gamma\in\mathcal{K}$ such that for each $M_{\mb{d}}\in\R_{\geq 0}$, the system \eqref{eq:dt_autonomous_dist} is safe with respect to the set $\mathcal{C}_{M_{\mb{d}}}$ defined as:
%     \begin{equation}
%         \mathcal{C}_{M_{\mb{d}}} \triangleq \{\mb{x}\in\R^n ~|~ h(\mb{x})\geq -\gamma(M_{\mb{d}})\},
%     \end{equation}
%     for all sequences of disturbances satisfying $\Vert\mb{d}_k\Vert\leq M_{\mb{d}}$ for all $k\in\mathbb{N}$.
% \end{definition}

% A system that is input-to-state safe gracefully degrades in the presence of the disturbances, such that the set rendered forward invariant grows continuously with the magnitude of the worst-case disturbance. ISSf is an analog of the well-known concept of Input-to-State Stability (ISS) for Lyapunov stable systems in the presence of disturbances \cite{sontag2008input}, which has also been adapted for DT systems \cite{jiang2001input}. The following proposition relates a DTBF and ISSf:

% \begin{proposition}\label{prop:issf_deterministic}
%     Let $\C\subset\R^n$ be the 0-superlevel set of a Lipschitz continuous function $h:\R^n\to\R$ with Lipschitz constant $\mathcal{L}_h\in\R_{\geq 0}$. If $h$ is a DTBF for \eqref{eq:dt_autonomous} on $\C$ for some $\alpha\in[0,1)$, then the system \eqref{eq:dt_autonomous_dist} is input-to-state safe with respect to the set $\C$ with $\gamma\in\mathcal{K}$ defined as:
%     \begin{equation}
%         \gamma(r) = \frac{\mathcal{L}_h r}{1-\alpha}.
%     \end{equation} 
% \end{proposition}
% \noindent A proof of this result is provided in Appendix \ref{pf:issf_deterministic}.



% Meanwhile, smaller $\alpha$ values lead to smaller expanded sets $\mathcal{C}_\gamma$, since, on the exterior of the set, smaller $\alpha$ values attempt to enforce faster convergence back to $\mathcal{C}$. 

%The second robustness property, ISSf, can also be compared for DTCBFs with varied $\alpha$. 

% This shows that smaller $\alpha$ values lead to smaller expanded sets $\mathcal{C}_\gamma$. This because, on the exterior of the set, smaller $\alpha$ values attempt to enforce faster convergence back to $\mathcal{C}$. 

% that will enable us to study the effect of unbounded disturbances. In particular, we will employ martingales to analyze the change in system safety over time and we will study the effects of Jensen's inequality on control applications. %, a bound which captures how random variables are effected by convex/concave mappings.

% For the remainder of this work we consider system \eqref{eq:dt_dyn}:
% \begin{align}
%     \mb{x}_{k+1} = \mb{F}(\mb{x}_k, \mb{u}_k) + \mathbf{d}_k, \quad \forall k \in \mathbb{N},  \label{eq:dt_dyn_dist2}
% \end{align}
% and corresponding closed-loop system \eqref{eq:dt_autonomous_dist}: 
% \begin{align}
%     \mb{x}_{k+1} = \mb{F}(\mb{x}_k, \mb{k}(\mb{x}_k)) + \mb{d}_k, \quad \forall k \in \mathbb{N}\label{eq:dt_autonomous_dist2}
% \end{align}
% Expanding beyond the bounded disturbance case, the disturbances $\mb{d}_k$ are now treated as independent and identically distributed random variables with potentially unbounded support.

% \ryan{not quite sure how to word this bit. We want to balance precision with clarity. }

% Consider a potentially unbounded sequence of random variables $H_0, H_1, \dots$ which take values in $\R$. This process is a martingale if it satisfies the martingale condition for all $k$: 
% \begin{align}
%     \E[H_{k+1} |H_{k:0} ] = H_k \textrm{ almost surely (ie, probability 1).}
% \end{align}
% \noindent where $H_{k:0}$ indicates the random variables $H_k$ through $H_0$. 

% In particular, this work will employ \textit{supermartingales} which are a generalization of martingales that are defined by an increase condition similar to the DTCBF decay constraint \eqref{eq:dtcbf_constraint}. 

% \begin{definition}[Supermartingale]
%     Let $H_K$ be a sequence of random variables for $k \in\mathbb{N}_{\geq 0}$ with finite expectation that take values in $\R$.  The process $H_k$ is a supermartingale if %$\E [\vert H_k \vert ] < \infty$ and 
%     \begin{align}
%         \E[~H_{k+1} ~|~  H_{k:0} ~] \leq H_k, \textrm{almost surely for all } k \geq 0. 
%         \label{eq:supermartingale}
%     \end{align} 
%     If, additionally, $H_k \geq 0$ for all $k \geq 0,$ then $H_k$ is a \textit{nonnegative supermartingale}.
% \end{definition}



% The safety guarantees provided by DTCBF-based controllers gracefully degrade in the presence of disturbances \cite{xu2015robustness, kolathaya2018input, chern_safe_2021, alan2022control}. This degradation has a strong dependence on the parameter $\alpha$, and will be important in constructing our formulation of safety for stochastic systems. We will describe the degradation of safety guarantees through two perspectives, beginning with the following definition:

% \begin{definition}[First Exit Time \cite{kushner1967stochastic}]
%     Let $\C\subset\R^n$ be the 0-superlevel set of a continuous function $h:\R^n\to\R$. For any initial condition $\mb{x}_0\in\R^n$, the first exit time of the system \eqref{eq:dt_autonomous_dist} with respect to $\C$ is given by:
%     \begin{equation}
%         K_{\rm esc}(\mb{x}_0) = \inf\{k\in\mathbb{N} ~|~ h(\mb{x}_k) < 0\}.
%     \end{equation}
% \end{definition}
% \noindent In general, systems with larger first exit times for a given initial condition $\mb{x}_0\in\mathcal{C}$ are considered to degrade more gracefully. Intuitively, this is because the system cannot be rendered unsafe by one instantaneous disturbance, but rather requires successive disturbances to become unsafe.

% The second perspective on the degradation of safety guarantees pertains to the set that is kept forward invariant in the presence of disturbances. DTCBF-based controllers induce a property known as Input-to-State Safety (ISSf) \cite{xu2015robustness, kolathaya2018input, alan2022control}, in which the set that is kept forward invariant is an expansion of the set $\C$ that grows relative to the magnitude of the disturbance. Intuitively, this is due to the fact that the DTBF inequality \eqref{eq:dtbf_constraint} requires the value of the DTBF to increase when it is negative (outside of the set $\C$). This effect balances with the disturbances to keep the system in a larger set in the state space. This perspective on the degradation of safety guarantees enables ISSf to serve as a powerful design tool when the original set $\C$ is designed with some margin \cite{alan2022control}. While we will not require a formal definition of ISSf in this work, it will conceptually appear as seen in the following example:


% \begin{example}\label{ex:1d_system} 
% \normalfont Consider the scalar DT nonlinear system:
% \begin{equation}
% \label{eq:ex_dyn}
%     x_{k+1} = x_k + 2 + u_k + \sigma d_k,
% \end{equation}
% and a safe set $\C$ specified as:
% \begin{equation}
% \label{eq:ex_safeset}
%     \C = \{x \in \R  ~|~ \underbrace{1-x^2}_{h(x)} \geq 0\}.
% \end{equation}
% The controller for the system is the \eqref{eq:dtcbfop} with $k_{\rm{nom}}(x) = 2+x$. We apply an independent and identically distributed disturbance  sampled from a uniform distribution $d_k \sim \mathcal{U}_{[-1, 1]}$ for $k\in\mathbb{N}$ with $\sigma = 0.01$ to the closed-loop system and simulate the system from %the initial condition 
% $x_0 = 0$. The value of $h(x_k)$ can be seen as a function of time for different values of 
% %the parameter 
% $\alpha$ in Fig.~\ref{fig:example}. For each value of $\alpha$, the simulation uses the same sequence of randomly generated disturbances in order to make the system behavior's dependence on $\alpha$ clear.

% We observe that the first exit time of the system increases as the value of $\alpha$ approaches $1$. This intuitively follows from the fact that larger values of $\alpha$ require the value of $h$ to make smaller decrements across time steps as given by \eqref{eq:dtbf_constraint}. 
% We next observe that while the system does leave the set $\C$, its distance from the set remains bounded, as described by ISSf. We see the system leaves the set $\C$ to a greater degree as the value of $\alpha$ increases, as indicated by the minimum value of $h$ across the simulation becoming more negative. Intuitively, this is because small values of $\alpha$ require the system to converge back to the set $\C$ very quickly, overpowering disturbances. For large values of $\alpha$, the system does not have to converge back to $\C$ quickly, and the disturbances can continue to pull the system away from $\C$. This apparent tradeoff between the first exit time and expansion of the set $\C$ will manifest when we develop a notion of stochastic safety.
% \end{example}

% \begin{figure}[t]
%     \centering
%     \includesvg[width=\linewidth]{figures/1D_alphas.svg}
%     \caption{\textbf{(Top)} Value of the DTBF $h$ defined in \eqref{eq:ex_safeset} along trajectories of the system \eqref{eq:ex_dyn} for different values of $\alpha$ ($\alpha_i = (3^i-1)/3^i$). \textbf{(Bottom Left)} The first exit time for different values of $\alpha$. Increasing the value of $\alpha$ leads to larger first exit times. \textbf{(Bottom Right)}  The minimum value of the DTBF $h$ along the simulation horizon for different values of $\alpha$. Increasing the value of $\alpha$ leads to a larger deviation of the system from the set $\C$.}
%     \label{fig:example}
% \end{figure}

% \noindent We will use this inequality in Theorem \ref{thm:kushner_main} to bound the probability that $h(\mb{x}_k) $ drops below a certain value. 
% \begin{proof}
%     Let $K$ the random variable which describes the first time when $H_k>\lambda$. Consider the event $A = \{ K < \infty  \} $. 
% \end{proof}

% In doing this we encounter Jensen's inequality which relates the expectation of the original distribution of $\mb{d}_k$ to the distribution of $h$ if $h$ is convex or convex. 

% We refer to $\psi \geq 0$ as the \textit{Jensen gap} if 
% \begin{align}
%     \psi = \vert \E[h(\mb{X})] - h(\E[\mb{X}]) \vert.
% \end{align}%holds with inequality holds with equality, then we refer to $\psi $ as the \textit{Jensen gap}. 

% We assume that the disturbance is bounded, such that there exists a $M_{\mb{d}}\in\R_{\geq 0}$ satisfying $\Vert\mb{d}_k\Vert \leq M_{\mb{d}}$ for all $k\in\mathbb{N}$.

% We will once again consider the system \eqref{eq:dt_dyn_dist} and its corresponding closed-loop system \eqref{eq:dt_autonomous_dist}, but we will assume that $\mb{d}_k$ is a sequence of independent and identically distributed random variables with (potentially unbounded) support on $\R^n$. 

% For these systems it is not necessarily possible to enforce safety for all $k \in \mathbb{N}$ with probability 1. For example, consider the case of keeping a gaussian distributed random variable inside of a finite interval. Due to the infinitely supported tails, the system will eventually leave the safe interval almost surely regardless of the control strategy.

% \preston{We might need to prove this as a proposition in the Appendix, it's trivial but might be non-obvious.}

% To do so, we reintroduce the DT stochastic invariance theorem of \cite{kushner1967stochastic,santoyo_verification_2019} and reframe it in the context of ISSf DTCBFs. We further provide a novel, (and, we believe, more intuitive) proof of these results, with the aim of making the mathematical tools available from martingale theory more accessible and generalizable.

%For stochastic safety we must draw connections between discrete-time Lyapunov first-exit times as studied by \cite{kushner1967stochastic} and reintroduced in the context of DTCBFs in \cite{santoyo_verification_2019}. We draw connections between these results and ISSf. 
% Furthermore, we re-state the proof from \cite{kushner1967stochastic} with more detail to help communicate this important result. 

% In the context of this result we assume that our state $\mb{x}_k $ is a stochastic process.  

% The theorem in \cite{kushner1967stochastic} provides bounds on a system's finite-time exit probability:

% Next we reframe the theorem in \cite[pg. 86]{kushner1967stochastic} to the context of DTCBFs and ISSf-like set expansions

    % The proof of this theorem wil rely on constructing a nonnegative super-martingale. The candidate martingale used here is taken from \cite{kushner1967stochastic} which, when the disturbance term is constant $(\varphi \triangleq M(1 - \alpha) - d)$ , can be rewritten using summation terms as: 
    % \begin{align}
    %     \widetilde{W}(\mb{x}_k, k) & = \underbrace{(M- h(\mb{x}_k))F(k, \theta)}_{\textrm{negate and rescale}}\underbrace{+  \varphi \left[ \sum_{i=k}^K F(i, \theta)   \right] }_{\textrm{cancel }d \textrm{ \& ensure nonnegativity}}\\
    %     \widetilde{F}(k, \theta) & = \left( \frac{\theta}{\theta - \varphi}\right)^k.
    % \end{align}
    % In summation form, this candidate martingale is of a form very similar to that used for stochastic safety analysis in \cite{steinhardt2012finite}, but the free variable $\theta \in \R_{>0}$ extends its utitility by allowing it to account for systems with $\alpha\neq 1$. 

    % First, we can use the geometric series identity for $\theta > 1$ $\left( \sum_{i=1}^k \theta^{i} = \frac{\theta(1- \theta^{k})}{1 - \theta}\textrm{ for } k\geq 1\right) $ to rewrite $W$ as: 
% \begin{align}
%     W(\mb{x}_k, k)  & = (M - h(\mb{x}_k))\theta^k+\varphi\left[\sum_{i=1}^K \theta^{i}-\sum_{i=1}^k \theta^{i}\right]\\
%     & =  (M - h(\mb{x}_k))\theta^k+ \frac{\varphi\theta}{\theta -1} \left[ \theta^K - \theta^k\right]
% \end{align}

% To verify that $W$ is a nonnegative supermartingale we must show that (1) it is nonnegative and (2) that it satisfies the supermartingale inequality.

% \eqref{eq:dt_autonomous_dist}, \eqref{eq:w_barrier_cond} follows from the barrier condition \eqref{eq:kushner_constraint}, and \eqref{eq:w_theta_const} adds an additional requirement that $\theta \leq \frac{1}{\alpha}.$
    % \begin{align}
    %     & \E[W(\mb{x}_{k+1}, k+1)]\nonumber\\
    %     & = (M - \E[h(\mb{x}_{k+1})])\theta^{k+1}+ \frac{\varphi\theta}{\theta -1} \left[ \theta^K - \theta^{k+1}\right] \\
    %     & \leq (M - \alpha h(\mb{x}_k) - d) \theta^{k+1}+ \frac{\varphi\theta}{\theta -1} \left[ \theta^K - \theta^{k+1}\right]\\
    %     & = \underbrace{\alpha \theta}_{\textrm{req.} \leq 1} (M - h(\mb{x}_k)) \theta^k + \frac{\varphi\theta}{\theta -1} \left[ \theta^K - \theta^{k+1}\right] + \varphi \theta^{k+1}\label{assp:theta_1}\\
    %     & \leq (M - h(\mb{x}_k) ) \theta^k +  \frac{\varphi\theta}{\theta -1}\left[\theta^K - \theta^{k+1} + \theta^k (\theta - 1) \right]  \\
    %     & = (M - h(\mb{x}_k))\theta^k+ \frac{\varphi\theta}{\theta -1} \left[ \theta^K - \theta^k\right]\\
    %     & = W_k.
        % & \leq (M - h(\mb{x}_k) ) \theta^k +  \frac{\varphi\theta}{\theta -1} \theta^K +\theta^{k+1} \left[   \frac{-\varphi\theta}{\theta -1} + \varphi \right]\\
        % & =  (M - h(\mb{x}_k) ) \theta^k +  \frac{\varphi\theta}{\theta -1} \theta^K -\theta^{k+1}    \frac{\varphi}{\theta -1} \\
        % & =  (M - h(\mb{x}_k) ) \theta^k -\theta^{k}    \frac{\varphi\theta}{\theta -1} +  \frac{\varphi\theta}{\theta -1} \theta^K  \\
        % &= W(\mb{x}_k, k). 
   % \end{align}
    % \noindent In line \eqref{assp:theta_1} added a constraint to $\theta$ and required that $\theta \leq \frac{1}{\alpha}$. 

    % \begin{definition}
%     Let $\mb{X}_k$ be a sequence of random variance that take values in $\R^n$ and consider a function $W: \R^n \times  \to \R $ where $\E[\vert W(\mb{X}_k, k ) \vert] < \infty  $ for $k \in \mathbb{N}_{\geq 0}$. The process $W(\mb{X}_k, k) $ is a supermartingale if: 
%     \begin{align}
%         \E[W(\mb{X}_{k+1}, k ) ~|~ \mb{X}_{k:0}] \leq W(\mb{x}_k, ) \textrm{ almost surely for all } k \in \mathbb{N}, 
%     \end{align}
%     where $\mb{X}_{0:k}$ indicates the random variables $\mb{x}_0, \dots, \mb{x}_k$. If additionally $W(\mb{X}_k, k) \geq 0 $ for all $k \in \mathbb{N}$, then 
%     % Let $\mb{X}_k$ be a Markov process (i.e. a random variable such that $p(\mb{X}_{k+1} | \mb{X}_k ) = p(\mb{X}_{k+1} | \mb{X}_{k:0}) ) $
% \end{definition} 

% \begin{definition}
%     Let $H_k$ be a sequence of random variables that take values in $\R$ and have finite expectation ($\mathbb{E} [ \vert H_k \vert ]<\infty$) 
%     for $k\in \mathbb{N}_{\geq 0}$. The process $H_k$ is a supermartingale if:
%     \begin{equation}
%     \label{eq:supermartingale}
%         \mathbb{E}[ H_{k+1} | H_{0:k}] \leq H_k~\textrm{almost~surely~for~all~}k\in\mathbb{N},
%     \end{equation}
%     where $H_{0:k}$ indicates the random variables $\left\{H_0, H_1, \ldots, H_k\right\}$. If, additionally, $H_k\geq 0$ for all $k\in\mathbb{N}$, $H_k$ is a nonnegative supermartingale. If the process increases in expectation, the process $H_k$ is a submartingale. If the inequality in \eqref{eq:supermartingale} holds with equality, the process $H_k$ is a martingale. 
% \end{definition}

% Choosing $\lambda $ such that $\min_{k\in \{ 0, \dots, K\}} r(k, \theta) = -\gamma$ (this is possible as $r(k,\theta) > 0$ with $\lambda = 0$), it must be true that: 
% For $k^* = \arg\min_{k \in \{0, \dots, K\}} r(k,\theta),$ this $\lambda $ would be: 
% \begin{align}
%     \lambda = \left( \gamma + M - \frac{\varphi \theta}{\theta -1}\right)\theta^{k^*} + \frac{\varphi \theta}{\theta-1} \theta^K. 
% \end{align}

%Using these results, we can now prove Theorem \ref{thm:kushner_main}. In particular, 

% \preston{I left off the ``proof'' environment here because it looks awkward and ``proof'' is in the section heading. We can probably reformat if we think ``proof'' and the square are important :)}

% \begin{align}
%     \mathcal{C} & \triangleq \left \{ \mb{x} \in \R^n \mid h(\mb{x}) \geq 0 \right \}, \\
%     % \textrm{Int}(\mathcal{C}) & \triangleq \left \{ \mb{x} \in \R^n \mid h(\mb{x}) > 0 \right \}, \\
%     % \partial \mathcal{C} & \triangleq \left \{ \mb{x} \in \R^n \mid h(\mb{x}) =  0 \right \}. 
% \end{align}

% Now, we seek to relate the level sets of the functions $W$ and $h$. In particular, using \eqref{eqn:wkgeomid}, we have that:
% \begin{align}
%      \max_{k \in \{0, \dots, K\}} & W_k - \lambda \nonumber \\
%     & = \max_{k \in \{0, \dots, K\}} -h(\mb{x}_k) \theta^k \\
%     & \quad \quad + \theta^k \left[ M - \frac{\varphi\theta}{\theta -1 } + \theta^{-k} \left( \frac{\varphi \theta}{\theta - 1}\theta^K - \lambda\right) \right], \nonumber \\
%     & \triangleq \max_{k \in \{0, \dots, K\}}  \theta^k\big(r(k, \theta, \lambda )-h(\mb{x}_k)\big), 
% \end{align}
% where we define:
% \begin{align}
%     r(k, \theta, \lambda) \triangleq M - \frac{\varphi\theta}{\theta -1 } + \theta^{-k} \left( \frac{\varphi \theta}{\theta - 1}\theta^K - \lambda\right).
% \end{align}
% \noindent Since $\theta > 1$, we have that $\max_{k \in \{0, \dots, K\}} W_k - \lambda > 0$ if and only if  $ \max_{k \in \{0, \dots, K\}} r(k, \theta, \lambda ) -h(\mb{x}_k) > 0$. In addition, we can trivially bound:
% \begin{align}
%      \max_{k \in \{0, \dots, K\}} &-h(\mb{x}_k) +  r(k, \theta, \lambda) \label{eq:minmaximp} \\
%      & \geq \max_{k \in \{0, \dots, K\}} -h(\mb{x}_k) + \min_{k \in \{ 0, \dots, K \}} r(k, \theta, \lambda). \nonumber \\
%      & = -\min_{k \in \{0, \dots, K\}} h(\mb{x}_k) + \min_{k \in \{ 0, \dots, K \}} r(k, \theta, \lambda ). \nonumber
% \end{align}
% Note that because $M>0$, for $\lambda = 0$, we have that $r(k,\theta, \lambda) > 0$ for all $k\in\{1,\dots,K\}$. Let us define:
% \begin{align}
%     \lambda_k = \left( \gamma + M - \frac{\varphi \theta}{\theta -1}\right)\theta^{k} + \frac{\varphi \theta}{\theta-1} \theta^K > 0, 
% \end{align}
% for which $r(k,\theta,\lambda_k) = -\gamma$. Because $r$ is a decreasing function of $\lambda$ for all $k\in\{1,\dots,K\}$ and $\theta\in(1,\infty)$, if $\lambda^* = \min_{k\in\{0,\dots,K\}}\lambda_k$, then $\min_{k\in\{0,\dots,K\}} r(k,\theta,\lambda^*) = -\gamma$.
% With this value of $\lambda^*$ we have from \eqref{eq:minmaximp} that:
% \begin{align}
%     \min_{k \in \{0, \dots, K\}} & h(\mb{x}_k) < -\gamma \nonumber \\  & \implies \max_{k \in \{0, \dots, K\}} -h(\mb{x}_k) +  r(k, \theta, \lambda^*) > 0, \nonumber \\
%     & \implies \max_{k \in \{0, \dots, K\}} W_k - \lambda^* > 0,
% \end{align}
% providing us with the desired conclusion:
% \begin{align}
%     P_u &=\P\left\{\min_{k \in \{0, \ldots, K\}} h(\mb{x}_k) < -\gamma\right\} \\&\leq \P \left\{ \max_{k \in \{0, \dots, K \}}  W_k > \lambda^* \right\} \leq \frac{W_0}{\lambda^*}.
% \end{align}

% & = \left( \frac{M - h(\mb{x}_0) }{M + \gamma }\right) \alpha^K +  \frac{M (1-\alpha) - \delta}{M + \gamma}\left( \frac{1- \alpha^K}{1 - \alpha } \right)\nonumber\\

%\geq \frac{\varphi \theta}{\theta -1} \theta^{K}. 

 %This ensures that $\argmin_{k \in \{0, \dots, K\}} r(k, \theta) $ occurs at $k^* = 0$ and 

     % \begin{remark}
    %     In the original proof presented in \cite{kushner1967stochastic} the values of $\theta$ used in Theorem \ref{thm:kushner_main} are said to minimize the probability bound without proof. Numerical simulations of the bounds suggests that this is true, but it remains to be proved rigorously. 
    % \end{remark}

    % \subsection{Finite-Time Safety using Chance Constraints}
    % \ryan{Add that you can analyze cvar controllers with our method. Remove chance constraint bounds}

    % Due to the use of the expectation and the restriction that $\alpha \in (0,1)$, the stochastic DTCBF condition in \eqref{eq:kushner_constraint} does not contain the standard chance constraint (which can be equivalently expressed as a Value-at-Risk constraint): 
    % \begin{align}
    %     \P \left \{ h(F(\mb{x}_k, \mb{u}_k) + \mb{d}_k) \geq -\gamma \right\} \geq p. \label{eq:chance_constraint}
    % \end{align}

    % One standard method for providing a bound for this system is using Boole's inequality (the union bound).

    % \begin{proposition}
    %     A system which satisfies \eqref{eq:chance_constraint} with $\mb{x}_0 \in\mathcal{C}_\delta$ must satisfy: 
    %     \begin{align}
    %         \P\left\{ \min_{k \in \{0, \dots, K\}} h(\mb{x}_k) \leq -\delta\right\} \leq K(1-p).
    %     \end{align}
    % \end{proposition}
    % \begin{proof}
    %     Apply Boole's inequality to the event $\cup_{k \in \{0, \dots, K\}} \{ h(\mb{x}_k) \leq - \delta  \}$
    % \end{proof}
    
    %  Since it is possible that there exist tighter bounds, this does not provide a direct method for comparison between systems constrained by chance constraints \eqref{eq:chance_constraint} and the stochastic DTCBF constraint \eqref{eq:kushner_constraint}. However, these bounds indicate a possible improvement in safety. 

    % Importantly, the stochastic DTCBF constraint \eqref{eq:kushner_constraint} results in a desirable bound without requiring knowledge of the disturbance distributions whereas chance-constrained methods require knowledge of the disturbance quantile.  

    % it is common 
%in the CBF literature 
% to include the CBF constraints in an optimization problem like the \ref{eq:dtcbfop} that enforces safety while achieving pointwise minimal deviation from a nominal controller $\mb{k}_\textrm{nom}: \R^n\times\mathbb{N}_{\geq 0} \to \R^m $ (e.g., a human operator or learning-based controller): 

% As noted in Section \ref{sec:background}, it is common to choose convex functions $h$ in order to ensure that \eqref{eq:dtcbf_op} is a convex program. 
%For continuous-time CBFs this optimization often results in well-studied convex optimization problems such as quadratic and second order cone programs that can be solved in real time \cite{ames2016control,dean_guaranteeing_nodate,cosner_measurement-robust_2021}. However, for discrete-time systems, this can result in much more complex optimization programs whose structure depends on the properties of $h$ and $F$. For this reason, several works assume that both $h$ and $F$ are linear with respect to the input \cite{ahmadi2019safe,agrawal2017discrete}. Other work has shown that the assumption that the input enters linearly is well suited for system whose true continuous dynamics are control-affine \cite{taylor_safety_2022}. 

% \begin{proposition}[Jensen's Inequality \cite{liao2018sharpening}]
%     Consider the function $h: \R^n \to \R$ and a random variable with finite expectation $\mb{X}$ that takes values in $\R^n$, 
%     \begin{align}
%         \begin{cases}
%         \textrm{if $h$ is convex, }& \textrm{then }  \E[h(\mb{X})] \geq h(\E[\mb{X}]),\\
%         \textrm{if $h$ is concave, } &\textrm{then }  \E[h(\mb{X})] \leq h(\E[\mb{X}]) ]
%         \end{cases} \label{prop:jensens}
%     \end{align}
% \end{proposition}

%satisfying it implies satisfaction of the expectation condition \eqref{eq:kushner_constraint} which allows us to apply the results of.% since the gap introduced by Jensen's inequality tightens the safety constraint. 

%(as is often assumed \cite{agrawal2017discrete,taylor_safety_2022,ahmadi2019safe,zeng2021safety}),

%Thus, in order to apply the results of Theorem \eqref{thm:kushner_main} to \eqref{eq:CE_dtcbf} we must reason about the effects of Jensen's inequality. 

%     References on trace bounding \cite{shebrawi2013trace,dragomir2018trace}.

% For convex function $\phi: \R^n \to \R$ 
% \begin{align}
%     \phi(x) & = \phi(\mu) + \nabla \phi(\mu)^\top (x- \mu) + \frac{1}{2}(x - \mu)^\top\nabla^2\phi(c) (x - \mu) \\
%     c & = \lambda x + (1- \lambda) \mu, \quad \lambda \in [0, 1] \\
%     \phi(x) & = \phi(\mu) + \nabla \phi(\mu)^\top ( x - \mu)  + \frac{1}{2}\textrm{tr} \left( \nabla^2 \phi(c) (x - \mu)(x - \mu)^\top \right)\\
%     & \leq \phi(\mu) + \nabla \phi(\mu)^\top ( x - \mu)  + \frac{1}{2}\textrm{tr} \left(  \nabla^2\phi(c) \right) \textrm{tr}\left( (x - \mu)(x - \mu)^\top \right)\\
%     & \leq \phi(\mu) + \nabla \phi(\mu)^\top ( x - \mu)  + \frac{1}{2}\underbrace{\sup_c \textrm{tr} \left(  \nabla^2\phi(c) \right)}_{H^*} \textrm{tr}\left( (x - \mu)(x - \mu)^\top \right)
% \end{align}

% \begin{align}
%     &\E [\phi(x) ] - \phi(\E[x]) = \int (\phi(x) - \phi(\mu) )p(x) dx \\
%     &\leq \int \left(\nabla \phi(\mu)^\top (x - \mu) + \frac{1}{2}(x - \mu)^\top \nabla^2\phi(c) (x - \mu)  \right) p(x) dx\\
%     &=  \int \textrm{tr}(\nabla^2 \phi(c) (x - \mu) (x - \mu) ^\top p(x) dx 
% \end{align}
% Can switch out for max eigenvalue of your Hessian. 

% we introduce an additional control parameter $\psi  \in \R_{\geq 0} $ which can be used to tighten the constraint and account for Jensen's Inequality in a Jensen-Aware dtCbf Controller (JACC): 

% In particular, by choosing a value of $\psi\in \R_{\geq 0}$ such that, for all $\mb{x}_{k+1} \in \R^n$, a concave function $h: \R^n \to \R $ and random variable $\mb{d}_k \sim \mathcal{D}$: 
% \begin{align}
%     \E[h(\mb{x}_{k+1}) +\mb{d}_k)] \geq h(\mb{x}_{k+1}) + \E[\mb{d}_k]) - \psi, \label{eq:jensen_gap}
% \end{align}
% \noindent we can undo the effects of Jensen's Inequality, which would allow us to apply the results of Theorem \ref{thm:kushner_main} to systems governed by a Jensen's-Aware CBF Controller (JACC) of the form: 
% \begin{align}
%     \mb{k}(\mb{x})^* = \argmin_{\mb{u} \in \R^m } \quad & \Vert \mb{u} - \mb{k}_{\textrm{nom}}(\mb{x}_k,k)  \Vert \label{eq:dtcbf_op_tighetened} \tag{JACC}\\ 
%     \textrm{s.t. } \quad & h(\mb{F}(\mb{x}_k, \mb{u}_k)+ \E[\mb{d}_k])  - \psi \geq \alpha h(\mb{x}_k). \nonumber
% \end{align}

% This theorem indicates a method by which we can analyze or account for the effects of the Jensen gap: 

% \ryan{This notation is a little wierd for the iid $\mb{d}_k$}

% \begin{corollary}
%     Consider the system \eqref{eq:dt_autonomous_dist2} and let $h:\R^n \to \R$ be a continuous convex function such that $\sup_{\mb{x} \in \R^n} h(\mb{x}) \leq M$ for some $M>0$.
%     %Additionally, let $\textrm{tr}(\textrm{cov}(\mb{d}_k)) \leq \sigma $ for some $\sigma>0$ and all $k \in \{ 0, \dots, N\} $.
%     Suppose that system \eqref{eq:dt_autonomous_dist2} satisfies: 
%     \begin{align}
%         h(\mb{F}(\mb{x}_k, \mb{k}(\mb{x}_k)) + \mathbb{E}[\mb{d}_k] ) - \psi \geq \alpha h(\mb{x}_k)  \label{eq:convex_h}
%     \end{align}
%     for some $\alpha \in (0,1)$, $\psi \in [0,  M(1-\alpha) ]$, and all $\mb{x}_k \in \R^n$. 

%     Then Theorem \ref{thm:kushner_main} holds with $\delta = \psi $. 
% \end{corollary}
% \begin{proof}
%     Inequality \eqref{eq:kushner_constraint} follows immediately from \eqref{eq:convex_h} and Jensen's inequality.
% \end{proof}

 % In this theorem we introduce a control parameter $\psi$ which can be used to account for the gap introduced by Jensen's inequality and add further robustness to the system. 

% \begin{theorem}\label{thm:kushner_jensen}
%     Let $\mb{x}_n, n \in \{0, \dots, N \}$ be a Markov process and $h:\R^n \to \R$ be a bounded continuous concave function such that $\sup_{\mb{x} \in \mathcal{X}} h(\mb{x}) \leq M$ for some $M>0$. Additionally assume that  $\sup_{\mb{x} \in \R^n} \Vert \lambda(\nabla^2 h(\mb{x})) \Vert \leq \lambda_{\max} $ for some $\lambda_{\max}>0$ and that the $\textrm{tr}(\textrm{cov}(\mb{d}_k)) \leq \sigma $ for some $\sigma>0$ and all $k \in \{ 0, \dots, N\} $.  Assume that $h$ satisfies: 
%     \begin{align}
%         h(\mb{F}(\mb{x}_k, \mb{u}_k) + \E[\mb{d}_k])\geq \alpha h(\mb{x}_k)+ \underbrace{\rho_k} \label{eq:dtcbf_jensen_constraint}
%     \end{align}
%     for all $\mb{x}_k \in \mathcal{X}$, some $\alpha \in (0,1)$, and $\rho_k \leq M(1-\alpha) $ for all $k \in \mathbb{N}$.  
    
%     For any $K \in \mathbb{N}_{\geq 0}$, the finite-time exit probability $P_u(K, \gamma)$ has the following bound:
%     \begin{align}
%         P_u \leq \frac{M - h(\mb{x}_0) + \theta ( F(K, \theta)- 1) }{(M + \gamma) F(K, \theta) }
%     \end{align}

%     Additionally, if $d_k \geq -\gamma (1 - \alpha) $ then the following alternative bound also applies: 
%     \begin{align}
%         P_u(K, \gamma) \leq 1 - \frac{h(\mb{x}_0) + \gamma }{M+\gamma}\prod_{i=0}^{K-1} \left(  \frac{M\alpha +\gamma +d_i}{M+ \gamma} \right) 
%     \end{align}
% \end{theorem}
% \begin{proof}
%     Lemma \ref{lm:jensen_gap}, ensures that \eqref{eq:dtcbf_jensen_constraint} implies that: 
%     \begin{align}
% \E[h(\mb{F})\mb{x}_k, \mb{u}_k) + \mb{d}_k \mid \mb{x}_k] \geq \alpha h(\mb{x}_k) + \rho_k - \frac{\lambda_\textrm{max}}{2}\textrm{tr}(\Sigma) 
%     \end{align}
%     By setting $d_k \triangleq \rho_k - \frac{\lambda_\textrm{max}}{2}\textrm{tr}(\Sigma) $ we can immediately apply Theorem \ref{thm:kushner_main}. 
% \end{proof}

% By setting $\rho_k \equiv 0 $ we establish a worst-case safety bound achieved when using controller \eqref{eq:dtcbf_after_jensens} in lieu of \eqref{eq:dtcbf_op}.  


% It is common in the usage of DT-CBFs to assume that $h \circ \mb{F}$ is a concave function with respect to $\mb{u}_k$. Since expectation is linear, this results in a convex constraint. However, despite the convexity of this constraint, it is still difficult to enforce since it requires that the distribution $\mb{x}_k$ be transformed by the potentially-nonlinear functions $h$ and $\mb{F}$. 

%  It is potentially easier to evaluate the expectation of the state $\mb{x}_k$ before evaluating the nonlinear functions $h$ and $\mb{F}$. This may occur in practical implementation if, for example, the mean output of the state estimator is used for control while the covariance is ignored. Unfortunately, assuming concavity with respect to $\mb{u}$ results in an inequality that does not provide sufficient strictnes to enforce the stochastic DT-CBF constraint in Theorem \ref{thm:1st_exit_time}. 

% References for flipping the Jensen bound \cite{liao2018sharpening,becker2012variance}. 

% If $h $ is concave, then Jensen's Inequality ensures that:  
% \begin{align}
%     h(\E[\mb{F}(\mb{x}_k, \mb{u}_k) ]) \geq \E[h(\mb{F}(\mb{x}_k, \mb{u}_k) ) ].                    
% \end{align}
% Therefore, enforcing $h(\E[\mb{F}(\mb{x}_k, \mb{u}_k)])\geq \alpha h(\mb{x}_k)$ does not allow us to use Theorem \ref{thm:kushner_main} to analyze our system. 

% We define our Jensen gap as: 
% \begin{align}
%     \varphi_\textrm{gap}(\mb{x}_k, \mb{u}_k)  \triangleq h(\E[\mb{F}(\mb{x}_k, \mb{u}_k) ]) - \E[h(\mb{F}(\mb{x}_k, \mb{u}_k) ) ] \geq 0 
% \end{align}

% The Jensen gap has been very thoroughly studied and bounds exist such as
% \begin{proposition}[Jensen Gap Bounds]
%     Some nice bound for the Jensen Gap.
% \end{proposition}

% When used in conjunction with Theorem \ref{thm:kushner_main}, we find the following result: 
% \begin{theorem}[\label{thm:kushner_jensen_main}]
%     Let $\mb{x}_n, n \in \{0, \dots, N \}$ be a Markov process and $h:\R^n \to \R$ be a bounded continuous function such that $\sup_{\mb{x} \in \mathcal{X}} h(\mb{x}) \leq M$ for some $M>0$. Assume that $h$ satisfies: 
%     \begin{align}
%         h(\mb{F}(\mb{x}_k, \mb{u}_k))   \geq \alpha h(\mb{x}_n) \label{eq:h_martingale}
%     \end{align}
%     for all $\mb{x}_n \in \mathcal{X}$ and some $\alpha \in (0,1)$. 
    
%     For some $N \in \mathbb{N}_{\geq 0}$, the finite-time exit probability $P_u(K, \gamma)$ has the following bound: 
%     \begin{align}
%         P_u(K, \gamma) \leq 1 - \frac{h(\mb{x}_0) + \gamma}{M + \gamma} \left( \frac{M\alpha + \gamma}{M+ \gamma}\right)^N 
%     \end{align}
% \end{theorem}
% \begin{proof}
% Same proof as Kushner, but now with a disturbance that is the result of a bound on the Jensen gap. 
% \end{proof}


%\clearpage

    %Let $\mb{x}_n$ be a Markov process for $ n \in \{0, \dots, N \}$ 

    %Additionally, let $\textrm{tr}(\textrm{cov}(\mb{d}_k)) \leq \sigma $ for some $\sigma>0$ and all $k \in \{ 0, \dots, N\} $.

     % Then, for any $K \in \mathbb{N}_{\geq 0}$, $\gamma \geq 0$, and $\psi \leq  \zeta_h(\mb{d}_k)  -\gamma(1 - \alpha)$: %the exit probability $P_u$ has the following bound:
    % \begin{align}
    %     P_u & \leq  \frac{M - h(\mb{x}_0 )}{M + \gamma } \alpha^K +  \frac{M (1 - \alpha) - \psi + \zeta_h(\mb{d}_k)}{M + \gamma}\sum_{i =1}^K\alpha^{i-1}  
    % \end{align}

    % Alternatively if $\psi \geq  \zeta_h(\mb{d}_k) -\gamma (1 - \alpha) $ then: 
    % \begin{align}
    %     P_u\leq 1 - \frac{h(\mb{x}_0) + \gamma }{M+\gamma}\left(  \frac{M\alpha +\gamma + \psi - \zeta_h(\mb{d}_k) }{M+ \gamma} \right)^K. 
    % \end{align}
    % \noindent Theorem \ref{thm:kushner_jensen} allows us to apply the probability bounds presented in Theorem \ref{thm:kushner_main} to systems which are governed by the \ref{eq:CE_dtcbf} and \ref{eq:jed} controllers. 

    % In this section we motivate our work on stochastic uncertainty with a deterministic example. When $\alpha \in (0,1]$ and $h(\mb{x}_k) > 0$ , the DT-CBF condition is more restrictive than the state constraint $h(\mb{x}_{k+1}) \geq 0 $ . However, in the disturbance-free case ($\Vert \mb{d}_k\Vert_\infty =0$), both ensure the safety of the system with respect to $\mathcal{C}$. This raises the question: 
% \begin{question}
% What is gained by restricting the safety constraint beyond $\alpha = 0$?
% \end{question}
% To analyze the robustness of these systems we start by considering an example which illustrates the effect of $\alpha$ on first exit times. 
% \begin{example}[Effects of $\alpha$ on First Exit Times] 
%     \normalfont
    % For $\mb{x}, \mb{u}, \mb{d} \in \R$, consider the system and set,

     % and the controller
    % \begin{align}
    %     \mb{k}(\mb{x}) = \argmin_{\mb{u} \in \R} & \Vert \mb{u} - (2 + \mb{x}_k) \Vert_2^2 \label{eq:example_controller} \\        
    %     \textrm{ s.t. } &  h(F(\mb{x}_k, \mb{u}_k)) \geq \alpha h(\mb{x}_k). \nonumber
    % \end{align}
    % where $\alpha \in [0, 1)$. 

        % For all $\mb{x}\in \mathcal{C}$ this system becomes unsafe in a single step when no input is applied. When $\mb{d}=0$, the controller \eqref{eq:example_controller} enforces the DTCBF constraint \eqref{eq:dtbf_constraint} and thus guarantees the safety of the system according to Theorem \eqref{thm:dtcbf}. When $\mb{d} > 0$, the system can become unsafe in finite time. 

    % Results of simulating this system for $d=0.05$ and $\alpha \in [0, 1)$ can be found in Fig. \ref{fig:example} where it is clear that larger $\alpha$ values led to larger first exit times.  



% As in \cite{steinhardt2012finite,santoyo_verification_2019} we consider a 1-dimensional linear system to verify our probability bounds: 
% \begin{align}
%     x_{k+1} = x_k  + 2 + \Delta t u_k + \sqrt{\Delta t} \sigma d_k
% \end{align}
% where $x_k, u_k\in \R $, $a \in \R$, $\sigma \in [0, 2] $, $\Delta t = 0.01$, and $d_k \sim \mathcal{N}(0, 1)$ is a standard gaussian-distributed disturbance. 

%This system is naturally very unsafe since nearly all safe initial conditions become unsafe in expectation after 1 time step if no control input is applied. 

% \begin{align}
%     h(\mb{F}(\mb{x}_k, \mb{u}_k))  \geq \alpha h(\mb{x}_k) + \underbrace{\sigma^2}_{\psi}, 
% \end{align}

% .which is the largest value of $\alpha$ that ensures feasibility for all $\mb{x} \in \R$. 
%Enforcing the tightest constraint yields a system which appears very stable to $x=0$, reducing $\alpha$ allows for more freedom to explore $\mathcal{C}$ but is coupled with looser safety bounds in theory and practice.

%\clearpage


% \section{RSS citations}

% Please make sure to include \verb!natbib.sty! and to use the
% \verb!plainnat.bst! bibliography style. \verb!natbib! provides additional
% citation commands, most usefully \verb!\citet!. For example, rather than the
% awkward construction 

% {\small
% \begin{verbatim}
% \cite{kalman1960new} demonstrated...
% \end{verbatim}
% }

% \noindent
% rendered as ``\cite{kalman1960new} demonstrated...,''
% or the
% inconvenient 

% {\small
% \begin{verbatim}x
% Kalman \cite{kalman1960new} 
% demonstrated...
% \end{verbatim}
% }

% \noindent
% rendered as 
% ``Kalman \cite{kalman1960new} demonstrated...'', 
% one can
% write 

% {\small
% \begin{verbatim}
% \citet{kalman1960new} demonstrated... 
% \end{verbatim}
% }
% \noindent
% which renders as ``\citet{kalman1960new} demonstrated...'' and is 
% both easy to write and much easier to read.
  
% \subsection{RSS Hyperlinks}

% This year, we would like to use the ability of PDF viewers to interpret
% hyperlinks, specifically to allow each reference in the bibliography to be a
% link to an online version of the reference. 
% As an example, if you were to cite ``Passive Dynamic Walking''
% \cite{McGeer01041990}, the entry in the bibtex would read:

% {\small
% \begin{verbatim}
% @article{McGeer01041990,
%   author = {McGeer, Tad}, 
%   title = {\href{http://ijr.sagepub.com/content/9/2/62.abstract}{Passive Dynamic Walking}}, 
%   volume = {9}, 
%   number = {2}, 
%   pages = {62-82}, 
%   year = {1990}, 
%   doi = {10.1177/027836499000900206}, 
%   URL = {http://ijr.sagepub.com/content/9/2/62.abstract}, 
%   eprint = {http://ijr.sagepub.com/content/9/2/62.full.pdf+html}, 
%   journal = {The International Journal of Robotics Research}
% }
% \end{verbatim}
% }
% \noindent
% and the entry in the compiled PDF would look like:

% \def\tmplabel#1{[#1]}

% \begin{enumerate}
% \item[\tmplabel{1}] Tad McGeer. \href{http://ijr.sagepub.com/content/9/2/62.abstract}{Passive Dynamic
% Walking}. {\em The International Journal of Robotics Research}, 9(2):62--82,
% 1990.
% \end{enumerate}
% %
% where the title of the article is a link that takes you to the article on IJRR's website. 


% Linking cited articles will not always be possible, especially for
% older articles. There are also often several versions of papers
% online: authors are free to decide what to use as the link destination
% yet we strongly encourage to link to archival or publisher sites
% (such as IEEE Xplore or Sage Journals).  We encourage all authors to use this feature to
% the extent possible.


%\clearpage

%\clearpage

% \subsection{Proposition \ref{prop:state_constraint_1st_exit_robustness}}
% \begin{proposition} \label{prop:state_constraint_1st_exit_robustness}
%     Consider the system \eqref{eq:dt_dyn}. For every $\mb{x}_0 \in \mathcal{C}$ there exists some dynamics $\mb{F}$ and controller $\mb{k}$ that satisfy \eqref{eq:dtcbf_constraint} with $\alpha = 0$ such that $K_\textrm{esc}=1$ for any $\Vert \mb{d}_0 \Vert > 0 $. 
% \end{proposition}
% \begin{proof}\label{pf:state_constraint_1st_exit_robustness}
%     The system satisfies $h(\mb{F}(\mb{x}_0, \mb{u}_0 )) \geq 0 $. Therefore, dynamics $\mb{F}$ such that $h(\mb{F}(\mb{x}_0, \mb{u}_0)) = 0 $ are admissible; the strictness of $\mathcal{C} \subset \R^n$ and continuous differentiability of $h$ imply that $\partial \mathcal{C}$ is non-empty. Since 0 is a regular value of $h$, for all $M>0$ there exists $\mb{d}_0 \in \R^n $ such that $\Vert \mb{d}_0 \Vert < M$ and $h(\mb{F}(\mb{x}_0, \mb{u}_0)  + \mb{d}_0)< 0$. 
% \end{proof}


% \subsection{Proposition \ref{prop:dt_cbf_constraint_1st_exit_robustness}}\label{pf:dt_cbf_constraint_1st_exit_robustness}
% \begin{proposition}\label{prop:dt_cbf_constraint_1st_exit_robustness}
%     Consider the system \eqref{eq:dt_dyn}. For every $\mb{x}_0 \in \textrm{Int}(\mathcal{C})$ there exists some disturbance  bound $M_\mb{d} >0$  such that if the dynamics-controller pair $(\mb{F}, \mb{k})$ satisfies \eqref{eq:dtcbf_constraint} with $\alpha >1$, then $\Vert \mb{d}_0 \Vert \leq M_\mb{d}$ implies that $K_\textrm{esc} >1$. 
% \end{proposition}
% \begin{proof}
%     $(\mb{F}, \mb{k})$ satisfy: $h(\mb{F}(\mb{x}_0, \mb{u}_0)) \geq \alpha h(\mb{x}_0) $ so: 
%     \begin{align}
%         h(\mb{x}_{1}) &\geq \min_{\Vert \mb{d}_0 \Vert \leq M_\mb{d} } h(\mb{F}(\mb{x}_0, \mb{u}_0) + \mb{d}_0 )\\
%         % & \geq h(\mb{F}(\mb{x}_0 , \mb{u}_0)) - \alpha h(\mb{x}_k) - \sup_{\Vert \mb{d}_k \Vert < \delta } \mathcal{L}_h \Vert \mb{d}_k \Vert \\
%         & \geq - \sup_{\Vert \mb{d}_k \Vert < M_\mb{d} } \mathcal{L}_h \Vert \mb{d}_k \Vert + \alpha h(\mb{x}_0) \\
%         & \geq - \mathcal{L}_h M_\mb{d} + \alpha h(\mb{x}_0) 
%     \end{align}
%     Where $\mathcal{L}_h$ is the Lipchitz constant of $h$ on the compact set $\textrm{cl}\left(B_{M_\mb{d}}(\mb{F}(\mb{x}_0, \mb{u}_0))\right) $.
%     % Applying this recursively results in: 
%     % \begin{align}
%     %     h(\mb{x}_{k}) \geq \alpha^k h(\mb{x}_0) - \sum_{\ell = 0}^{k-1} \alpha^{\ell} \mathcal{L}_h \delta.
%     % \end{align}
%     % where we let $0^0=1$. 
%     % Then 
%     % \begin{align}
%     %     K_\textrm{esc}(\alpha, \mb{x}_0) \geq  \max  \left\{ k \in \mathbb{N}_{\geq 1} \mid \alpha^k h(\mb{x}_0) \geq  \sum_{\ell = 0 }^{k - 1} \alpha^\ell \mathcal{L}_h \delta \right\}.
%     % \end{align} 
%     Choose $M_\mb{d} = \frac{\alpha h(\mb{x}_0)}{\mathcal{L}_h} > 0 $ to ensure that $K_\textrm{esc} > 1$. 
%     %and the system is guaranteed to be safe with respect to $\mathcal{C}$ for all $k \in \{ 0, \dots, K_\textrm{cbf}(\alpha, \mb{x}_0) \}$ since $k \in \{ 0 , \dots, K_\textrm{cbf}(\alpha) \} \implies  \alpha^k h(\mb{x}_0) - \sum_{\ell = 0}^{k-1} \alpha^{\ell} \mathcal{L}_h M \geq 0 \implies h(\mb{x}_k) \geq 0  $. 
% \end{proof}

% \subsection{Proposition \ref{prop:issf_deterministic}}

% \begin{proposition*}\label{prop:issf_deterministic}
%     Consider system \eqref{eq:dt_dyn}. If $h$ is Lipschitz continuous with constant $\mathcal{L}_h > 0 $, the dynamics-controller pair $(\mb{F}, \mb{k}) $ satisfies  \eqref{eq:dtcbf_constraint} for some $\alpha \in [0,1)$, and $\Vert \mb{d}_k\Vert \leq M_\mb{d}$ for some $M_\mb{d} >0$, then 
%     %with Lipschitz constant $L_h > 0$ and disturbance bound $\delta > 0 $ is ISSf with: 
%         $\mathcal{C}_\gamma = \left \{ \mb{x} \in \R^n \mid h (\mb{x}) \geq  \frac{-\mathcal{L}_h M_\mb{d} }{(1- \alpha) } \right \} $
%     is forward invariant (ie, safe). 
% \end{proposition*}
% \begin{proof} \label{pf:issf_deterministic}
%     \begin{align}
%         &h(\mb{F}(\mb{x}_k, \mb{u}_k))  \geq \alpha h(\mb{x}_k) \\
%         \implies &h(\mb{F}(\mb{x}_k, \mb{u}_k) + \mb{d}_k) + \mathcal{L}_h M_\mb{d}  \geq \alpha h(\mb{x}_k) 
%     \end{align}
%     Then this implies that for $h(\mb{x}_k) = \frac{- \mathcal{L}_h \delta }{(1 - \alpha) }$, 
%     \begin{align}
%         h(\mb{F}(\mb{x}_k, \mb{u}_k) \geq - \frac{\mathcal{L}_h \delta}{1 - \alpha }
%     \end{align}
%     So $\mathcal{C}_\gamma$ is safe with $\gamma(M_\mb{d})  = \frac{\mathcal{L}_h M_\mb{d}}{1 - \alpha }$. 
% \end{proof}

% \begin{lemma*}\label{lm:jensen_gap}
% Consider the concave function $h: \R^n\to \R$ with $\sup_{\mb{x} \in \R^n} \Vert \lambda(\nabla^2 h(\mb{x})) \Vert \leq \lambda_{\max} $ for some $\lambda_{\max}>0$ and a random variable $\mb{X}$ with finite expectation $\bs{\mu} \in \R^n $ and covariance $\Sigma \in \R^{n\times n}$. Then 
%     \begin{align}
%         \E[h(\mb{X})] \geq h(\E[\mb{X}]) - \frac{\lambda_\textrm{max}}{2} \textrm{tr}(\Sigma)
%     \end{align}
%     where $\lambda: \R^{n\times n} \to \R^n$ is a function which returns the eigenvalues of its argument. 
% \end{lemma*}




% \subsection{Theorem \ref{thm:1st_exit_time}}[\label{pf:1st_exit_time}]

% \begin{proof}
%     \begin{align}
%         K_\textrm{cbf}(0, \mb{x}_0) & = \sup  \left\{ k \in \mathbb{N}_{\geq 0} \mid 0^k h(\mb{x}_0) \geq  \sum_{\ell = 0 }^{k - 1} 0^\ell \mathcal{L}_h M \right\}\\
%         & = \sup  \left\{ 0  \right\} 
%     \end{align}
%     where we again let $0^0 = 1$. $K_\textrm{cbf}(0, \mb{x}_0) $ is always less than 1 since $0  < \mathcal{L}_hM  $ and always greater than or equal to 0 since $h(\mb{x}_0) \geq 0 $. $K_\textrm{cbf}(\alpha, \mb{x}_0)$ is always greater than or equal to 0 since $h(\mb{x}_0) \geq 0$, but may be greater than zero if $\alpha h(\mb{x}_0) \geq \mathcal{L}_h M$. Thus, $K_\textrm{cbf}(0) \leq K_\textrm{cbf}(\alpha)$. 
% \end{proof}

==> variable_phi_proof.tex <==


\begin{proof}
    To prove this theorem, we will rely on Ville's Inequality. In order to do that we first construct, a nonnegative super martingale. 
    For this purpose consider the candidate function $W: \R^n \times \mathbb{N}_\geq 0 \to \R^n  $: 
    \begin{align}
        W(\mb{x}_k, k) & \triangleq \underbrace{( M - h(\mb{x}_k)) F(k, \theta) } _{\textrm{negate and rescale}} - \theta \underbrace{F(k,\theta)}_{\textrm{cancel }d_i} + \underbrace{\theta F(K,\theta) }_{\textrm{ensure nonegativity}} \\ %\underbrace{\frac{\gamma + M}{K^N}}_{\textrm{ensure nonnegativity}}.\
        F(k, \theta) & \triangleq  
        \begin{cases}
            \prod_{i=0}^{k-1} \frac{\theta }{\theta - \varphi_i }, & k > 1\\
            1, & k = 1
        \end{cases}    \end{align}
    Where $\varphi_i \triangleq  M(1-\alpha) - d_i $, $\overline{\varphi}\triangleq \max_{i \in [0,K]} \varphi_i $, and $\theta \in \R_{>\overline{\varphi}}$ is a free variable which will be used later to optimize the bound on $P_u$. Nonegativity of $\varphi_i$ is implied by the assumption that $d_i \leq M(1- \alpha) $.
    % Inspired by the geometric series identity, $\sum_{i=k}^K a \theta^{1-i)} = \frac{a\theta (\theta^{-k} - \theta^{-N}) }{\theta - 1}$ for any $a \in \R$,  we approximate $\Tilde{W}$ as $W$: 
    % \begin{align}
    %     W(\mb{x}_k, k) &= F(k, \theta) V(x_k) - \theta F(k, \theta) + \theta F(K, \theta)\\
    %     F(k, \theta) & = 
    %     \begin{cases}
    %         \prod_{i=0}^{k-1} \frac{\theta }{\theta - \left[ M(1-\alpha) - d_i\right] }, & k > 1\\
    %         1, & k = 1
    %     \end{cases}
    % \end{align}
    
    % Substituting the identity for a finite geometric series,    results in: 
    % \begin{align}
    %     & W(\mb{x}_n, n) \\
    %     & = \frac{M - h(\mb{x}_n)}{\alpha^n} + M(1-\alpha)\left( \frac{\alpha^{-N}-1}{1 - \alpha} - \frac{\alpha^{-n}-1}{1- \alpha}\right) \\
    %     & = \frac{M - h(\mb{x}_n)}{\alpha^n} + M \left( \alpha^{-N} - \alpha^{-n} \right) \\
    %     & = -\frac{h(\mb{x}_n)}{\alpha^n} + M\alpha^{-N}
    % \end{align}
    
    We first show that it is nonnegative. Since $h(\mb{x}) \leq M$ for all $\mb{x}$, nonnegative is assured since $\theta \geq \overline{\varphi}$ implies that $F(k, \theta) $ is positive and that $F(k, \theta) $ increases as $k$ increases. 
    
    Next we must show that $W(\mb{x}_n, n)$ satisfies the super-martingale inequality: 
    \begin{align}
        & \mathbb{E}[W(\mb{x}_{k+1}, k+1) ~|~ (\mb{x}_k, k)] \nonumber \\
        & = (M- \E[h(\mb{x}_{k+1})~|~ x_k])F(k+1, \theta)   - \theta F(k+1, \theta) + \theta F(K, \theta)\\
        & \leq  (M - \alpha h(\mb{x}_k) - d_k )\frac{\theta}{\theta- \varphi_k} - \theta F(k+1, \theta) + \theta F(K, \theta)\\
        & \leq  \frac{\alpha \theta  (M -  h(\mb{x}_k)) + \theta \varphi_k }{\theta - \varphi_k} F(k , \theta)  - \theta F(k+1, \theta) + \theta F(K, \theta)
    \end{align}
    Here we choose $\theta \geq \varphi_k / (1 - \alpha) $ such that $\alpha \theta / (\theta - \varphi_k) \leq 1  $. 
    \begin{align}
        & \leq (M-h(\mb{x}_k))F(k, \theta)  + \theta F(K, \theta) - \theta F(k, \theta) \frac{\theta}{\theta - e_{k}} + \frac{\theta \varphi_k}{\theta - \varphi_k}F(k)\\
        & =  (M-h(\mb{x}_k))F(k, \theta)  + \theta F(K, \theta) - \theta F(k, \theta ) \left( \frac{\theta}{\theta - e_{k}} - \frac{ \varphi_k}{\theta - \varphi_k}\right) \\
        & = (M-h(\mb{x}_k))F(k, \theta)  - \theta F(k, \theta) - \theta F(K, \theta) 
    \end{align}
    \noindent     Thus, if $\theta \geq \varphi_k/(1-\alpha) $, then $W(\mb{x}_k, K) $ is a nonnegative super-martingale. 
    %Note that since $\alpha \in (0,1)$ $\gamma\geq 0$, and $M>0$,  $ [\alpha, \frac{\alpha M + \gamma }{M + \gamma  } ] $ is non-empty. 
    
    Since we have shown that $W(\mb{x}_k, K) $ is a nonnegative super-martingale, we can apply Ville's Inquality: 
    \begin{align}
        \mathbb{P}\left\{\max_{0\leq n \leq N} W(\mb{x}_n, n) \geq \lambda \right\}\leq \frac{M - h(\mb{x}_0) - \theta + \theta F(K, \theta)  }{\lambda}
    \end{align}
    
    Now we must relate level sets of $W(\mb{x}_n, n) $ to level sets of $h$. In particular, to bound $P_u$ we require that $\min_{n \in \{0, \dots, N\} } h(\mb{x}_n) \leq -\gamma $ implies that $\max_{n \in \{0, \dots, N\}}W(\mb{x}_n, n) \geq \lambda $. 
    \begin{align}
        &\max_{k \in \{0, \dots, N\}}  W(\mb{x}_n, n) -\lambda \nonumber\\
        & = \max_{k \in \{0, \dots, N\}} - h(x_k) F(k , \theta)  + \left( (M -\theta) F(k, \theta) + \theta F(K, \theta) - \lambda \right)  \\
        & \geq  -\min_{k \in \{0, \dots, N\}} h(\mb{x}_k)F(k, \theta)  \\
        & \quad + F(k, \theta) \underbrace{\left( (M -\theta)  + \frac{1}{F(k, \theta) }(\theta F(K, \theta) - \lambda) \right)}_{r(k, \theta ) \triangleq} 
    \end{align}
    To lowerbound this we seek to choose $\theta$ and $\lambda$ such that $\min_{k} r(k, \theta) \geq  -\gamma$

    \begin{align}
        r(k^*, \theta) & = (M -\theta)  + \frac{1}{F(k^*, \theta) }(\theta F(K, \theta) - \lambda) = -\gamma\\
        \lambda & = (M + \gamma - \theta) F(k^*, \theta) + \theta F(K, \theta) 
    \end{align}

    Since we previously restricted $\theta \geq \frac{\overline{\varphi} }{(1 - \alpha) }$, picking $\theta \geq \max\left\{ \frac{\overline{\varphi} }{(1 - \alpha) }, M + \gamma  \right\} $ ensures that: 
    \begin{align}
        \lambda & \leq \theta F(K, \theta). 
    \end{align}
    Additionally, this implies that $k^* = K$ minimizes $r(k, \theta)$ which yields the probability bound: 
    \begin{align}
        P_u \leq \frac{M - h(\mb{x}_0) - \theta + \theta F(K, \theta)  }{(M + \gamma ) F(K, \theta)  }, 
    \end{align}
    which is decreases as $\theta$ decreases, so we pick $\theta = \max\left\{ \frac{\overline{\varphi} }{(1 - \alpha) }, M + \gamma  \right\} $ to achieve our general probability bound. 

    Additionally, consider the case where $\left[ \frac{\varphi}{(1 - \alpha) }, M + \gamma \right]$ is a non-empty set. Choosing $\theta $ in that set yields: 
    \begin{align}
        \lambda \geq \theta F(K, \theta). 
    \end{align}
    \noindent which implies that $k^*=0$ minimizes $r(k , \theta) $ which yields the probability bound: 
    \begin{align}
        P_u \leq \frac{M - h(\mb{x}_0) + \theta ( F(K, \theta)  -1)  }{(M + \gamma ) + \theta( F(K, \theta) -1)   }
    \end{align}
    \noindent which decreases as $\theta$ increases, so we pick $\theta = M + \gamma$ to achieve our general probability bound. 

    

    % Thus 
    % \begin{align}
    %     P_u &\leq  \frac{M - h(\mb{x}_0) - \theta + \theta F(K, \theta)  }{(M + \gamma - \theta) F(k^*, \theta) + \theta F(K, \theta) },\\
    %     & = \frac{M - h(\mb{x}_0) + \theta( F(K, \theta) -1)   }{(M + \gamma ) F(k^*, \theta) + \theta (F(K, \theta) - F(k^*, \theta))  }
    % \end{align}




    % Consider 2 cases $\uderline{d} > \gamma(1-\alpha) $ and $\underline{d} \geq \gamma(1- \alpha) $. 

    % \textbf{Case 1: } $\underline{d} > \gamma( 1- \alpha) $ so $\overline{\varphi} < (M + \gamma)(1- \alpha)  $. In this case 
    % \begin{align}
    %     \lambda & = (M + \gamma - \theta) F(k^*, \theta) + \theta F(K, \theta) 
    % \end{align}
    
    
    \end{proof}


